Faster Spectral Sparsification in Dynamic Streams

Graph sketching has emerged as a powerful technique for processing massive graphs that change over time (i.e., are presented as a dynamic stream of edge updates) over the past few years, starting with the work of Ahn, Guha and McGregor (SODA'12) on graph connectivity via sketching. In this paper we consider the problem of designing spectral approximations to graphs, or spectral sparsifiers, using a small number of linear measurements, with the additional constraint that the sketches admit an efficient recovery scheme. Prior to our work, sketching algorithms were known with near optimal $\tilde O(n)$ space complexity, but $\Omega(n^2)$ time decoding (brute-force over all potential edges of the input graph), or with subquadratic time, but rather large $\Omega(n^{5/3})$ space complexity (due to their reliance on a rather weak relation between connectivity and effective resistances). In this paper we first show how a simple relation between effective resistances and edge connectivity leads to an improved $\widetilde O(n^{3/2})$ space and time algorithm, which we show is a natural barrier for connectivity based approaches. Our main result then gives the first algorithm that achieves subquadratic recovery time, i.e. avoids brute-force decoding, and at the same time nontrivially uses the effective resistance metric, achieving $n^{1.4+o(1)}$ space and recovery time. Our main technical contribution is a novel method for `bucketing' vertices of the input graph into clusters that allows fast recovery of edges of high effective resistance: the buckets are formed by performing ball-carving on the input graph using (an approximation to) its effective resistance metric. We feel that this technique is likely to be of independent interest.

==> macros.tex <==
%\documentclass[letterpaper,12pt]{book}
%	%TODO: book -> amsbook
%	%\pdfoutput=1
%	%\usepackage[utf8]{inputenc}
%	\usepackage{amsfonts, amsmath, amssymb, amsthm}
%	\usepackage{bbm}
%	\usepackage{thmtools}
%	\usepackage{algpseudocode}
%	\usepackage{graphicx}
%	\usepackage{stmaryrd}
%	\usepackage[show]{ed}
%	\usepackage{version}
%	\usepackage[small]{complexity}
	\usepackage[normalem]{ulem}
%	\usepackage{xspace}
%	\usepackage{lmodern}
%	\usepackage{nicefrac}
%	%\usepackage{authblk}
%	\usepackage[noadjust]{cite}
%	\usepackage[margin=1in]{geometry}
%	\usepackage{microtype}
%	\usepackage{nag}
%	\usepackage{nth}
%	\usepackage{intcalc}
%	\usepackage{background}
%	\usepackage{tocbibind}
%	\backgroundsetup{pages=all,color=black!100,angle=0,placement=top,vshift=-.2in,scale=1}
%	\usepackage[hyphens]{url}
%	\usepackage[pdftex,pagebackref=true,colorlinks=true,linkcolor=blue]{hyperref}
%	\usepackage{algorithm}
%
	% https://tex.stackexchange.com/questions/106714/stmaryrd-and-boldsymbol-avoid-warnings
	%\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}

	\PackageWarning{miforbes}{overfullrule enabled}
	% TODO: make this a switch
	\overfullrule=1mm

	% tikz now barfs at me, something about redefined dollarsigns
	% fix from https://tex.stackexchange.com/questions/165929/semiverbatim-with-tikz-in-beamer
	\makeatletter
	\global\let\tikz@ensure@dollar@catcode=\relax
	\makeatother

	% need to make thmtools' \listoftheorems give better spacing
	% from https://tex.stackexchange.com/questions/53774/horizontal-spacing-issue-in-listoftheorems-using-amsthm-thmtools
	\makeatletter
	\renewcommand\thmt@listnumwidth{4.3em}
	\makeatother

	\newcommand{\anote}[1]{\ednote{(Amir) #1}}
	\newcommand{\mfnote}[1]{\ednote{(miforbes) #1}}
	\newcommand{\TODO}[1]{\PackageWarning{miforbes}{#1}\texttt{TODO: #1}}
	\newcommand{\TODOsloppy}[1]{\PackageWarning{miforbes-sloppy}{sloppy}\sloppy #1}

	\numberwithin{equation}{section}
	\declaretheoremstyle[bodyfont=\it,qed=$\qedsymbol$]{noproofstyle} 

	\theoremstyle{plain}
	% things I prove
	% wp means things are too obvious to prove (eg, with lemma or corollary)
	\declaretheorem[numberlike=equation]{theorem}
	\declaretheorem[unnumbered,name=Theorem]{theorem*}
	\declaretheorem[numberlike=equation,name=Theorem,style=noproofstyle]{theoremwp}
	\declaretheorem[numberlike=equation,name=Theorem,style=noproofstyle]{theoremwp*}

	\declaretheorem[numberlike=equation]{lemma}
	\declaretheorem[unnumbered,name=Lemma]{lemma*}
	\declaretheorem[numberlike=equation,name=Lemma,style=noproofstyle]{lemmawp}
	\declaretheorem[unnumbered,name=Lemma,style=noproofstyle]{lemmawp*}
	
	\declaretheorem[numberlike=equation]{corollary}
	\declaretheorem[unnumbered,name=Corollary]{corollary*}
	\declaretheorem[numberlike=equation,name=Corollary,style=noproofstyle]{corollarywp}
	
	\declaretheorem[numberlike=equation]{proposition}
	\declaretheorem[unnumbered,name=Proposition]{proposition*}
	\declaretheorem[numberlike=equation]{claim}
	\declaretheorem[unnumbered,name=Claim]{claim*}
	\declaretheorem[numberlike=equation]{conjecture}
	\declaretheorem[unnumbered,name=Conjecture]{conjecture*}

	\declaretheorem[numberlike=equation,style=noproofstyle]{construction}
	\declaretheorem[unnumbered,name=Construction=noproofstyle]{construction*}

	% things I didn't prove
	\declaretheorem[numberlike=equation,name=Theorem]{theorem-cited}
	\declaretheorem[numberlike=equation]{fact}

	%\theoremstyle{definition}
	\declaretheoremstyle[qed=$\lozenge$,bodyfont=\it]{defstyle} 
	\declaretheorem[numberlike=equation,style=defstyle]{definition}
	\declaretheorem[unnumbered,name=Definition,style=defstyle]{definition*}
	\declaretheorem[numberlike=equation,style=defstyle]{example}
	\declaretheorem[unnumbered,name=Example,style=defstyle]{example*}
	\declaretheorem[numberlike=equation,style=defstyle]{notation}
	\declaretheorem[unnumbered,name=Notation,style=defstyle]{notation*}
	\declaretheorem[numberlike=equation,style=defstyle]{question}
	\declaretheorem[unnumbered,name=Question,style=defstyle]{question*}

	%\theoremstyle{remark}
	\declaretheoremstyle[qed=$\lozenge$,bodyfont=\it]{rmkstyle} 
	\declaretheorem[numberlike=equation,style=rmkstyle]{remark}
	\declaretheorem[unnumbered,name=Remark,style=rmkstyle]{remark*}

	\renewcommand{\subsectionautorefname}{Subsection}
	\renewcommand{\sectionautorefname}{Section}
	\renewcommand{\chapterautorefname}{Chapter}
	\newcommand{\algorithmautorefname}{Algorithm}
	\renewcommand{\proofname}{Proof:}

	\newcommand{\demph}[1]{\textbf{#1}}

	\newcommand{\naive}{na\"{\i}ve\xspace}

	% miforbes macros

	%       [
	\newcommand{\ocint}[2]{\ensuremath{(#1,#2]}}%)
	%       (
	\newcommand{\coint}[2]{\ensuremath{[#1,#2)}}%]
	\newcommand{\ccint}[2]{\ensuremath{[#1,#2]}}%)
	\newcommand{\ooint}[2]{\ensuremath{(#1,#2)}}%)
	\newcommand{\zr}[1]{{\llbracket {#1}\rrbracket}}
	\newcommand{\ind}[1]{\mathbbm{1}_{#1}}
	%while I like the idea of Iverson's bracket, it seems hard to come up with a bracket not used for other purposes.  Perhaps more seriously, there is the issue that given a predicate P, we want a function f_P(x) that takes as input x and tests if P is true on x.  This functional notation is crucial for situations where it is important to distinguish the inputs from the specification of the function.  eg, if we have a family of sets S_i, and want to test the condition "x\in S_i", it is wholly unclear whether we should regard this as a function of i, a function of x, or a function of both.  Perhaps this ambiguity is okay, but I feel unsettled by it.
	%\newcommand{\ind}[1]{\llb #1\rrb}
	\newcommand{\bits}{\ensuremath{\{0,1\}}}

	\newcommand{\llb}{\llbracket}
	\newcommand{\rrb}{\rrbracket}
	\newcommand{\la}{\langle}
	\newcommand{\ra}{\rangle}
	\newcommand{\from}{\leftarrow}

	\DeclareMathOperator{\ideg}{ideg}
	\DeclareMathOperator{\rank}{rank}
	\DeclareMathOperator{\trdeg}{tr-deg}
	\DeclareMathOperator{\sgn}{sgn}
	\DeclareMathOperator{\adj}{adj}
	\DeclareMathOperator{\perm}{perm}
	\DeclareMathOperator{\spn}{span}
	\DeclareMathOperator{\im}{im}
	\DeclareMathOperator{\cfspn}{coeff-span}
	\DeclareMathOperator{\cspn}{col-span}
	\DeclareMathOperator{\rspn}{row-span}
	\DeclareMathOperator{\chara}{char}
	\DeclareMathOperator{\tr}{tr}
	\DeclareMathOperator{\supp}{Supp}
	\DeclareMathOperator*{\argmax}{arg\,max}
	\DeclareMathOperator*{\argmin}{arg\,min}
	\DeclareMathOperator{\trexp}{\lfloor\exp\rfloor}
	%https://tex.stackexchange.com/questions/34818/declaremathoperator-wont-take-arguments
	\newcommand{\coeff}[1]{{\mathrm{Coeff}}_{#1}}
	%TODO: make mathop not do limits
	\newcommand{\homp}[1]{H_{#1}}
	\DeclareMathOperator{\GL}{GL}
	\let\SL\undefined
	\DeclareMathOperator{\SL}{SL}
	\DeclareMathOperator{\KL}{KL}
	\DeclareMathOperator{\LM}{LM}
	\DeclareMathOperator{\LT}{LT}
	\DeclareMathOperator{\jac}{Jac}
	\DeclareMathOperator{\grad}{\nabla}
	\DeclareMathOperator{\ent}{H}
	\DeclareMathOperator{\bent}{h}
	\DeclareMathOperator{\Ex}{\E}
	\DeclareMathOperator{\Ext}{Ext}
	\DeclareMathOperator{\stdistop}{\Delta}
	\newcommand{\stdist}[2]{\Delta_{\mathrm{st}}(#1;#2)}
	\newcommand{\stdistp}[2]{\Delta_{\mathrm{st}}\left(#1;#2\right)}
	\newcommand{\rinv}{\ensuremath{\F[\vX]^{\GL_n(\F)}}}
	\newcommand{\st}{\ensuremath{\ |\ }}
	\newcommand{\Pow}{\ensuremath{\wedge}}

	% derivatives
	\newcommand{\hasse}{\partial}
	\newcommand{\hasseu}{\hasse_{\vu^a}}
	\newcommand{\hassev}{\hasse_{\vv^b}}
	\newcommand{\hasses}{\boldsymbol{\hasse}}
	\newcommand{\shiftx}{\boldsymbol{\vx}}
	\newcommand{\shifty}{\boldsymbol{\vy}}
	\newcommand{\coeffs}[1]{{\mathbf{Coeff}}_{#1}}
	\newcommand{\evals}[1]{{\mathbf{Eval}}_{#1}}
	\newcommand{\spaceplus}{\boldsymbol{+}}
	\newcommand{\spacetimes}{\boldsymbol{\cdot}}

	\newcommand{\floor}[1]{{\lfloor{#1}\rfloor}}	
	\newcommand{\floorp}[1]{{\left\lfloor{#1}\right\rfloor}}	
	\newcommand{\ceil}[1]{{\lceil{#1}\rceil}}	
	\newcommand{\ceilp}[1]{{\left\lceil{#1}\right\rceil}}	
	\newcommand{\nc}[1]{{\la #1\ra}}
	\newcommand{\ncp}[1]{{\left\la #1\right\ra}}
	\newcommand{\ps}[1]{{\llb #1\rrb}}
	\newcommand{\subsets}[1]{2^{#1}}
	\newcommand{\kl}[2]{\KL({#1}\|{#2})}
	\newcommand{\klp}[2]{\KL\left({#1}\middle\|{#2}\right)}
	\newcommand{\klb}[3]{\KL_{#1}({#2}\|{#3})}
	\newcommand{\klbp}[3]{\KL_{#1}\left({#2}\middle\|{#3}\right)}
	\newcommand{\logp}{\log^+}
	\newcommand{\lgp}{\lg^+}
	\newcommand{\lnp}{\ln^+}

	% blackboard board
	\renewcommand{\E}{\mathbb{E}}
	\renewcommand{\C}{\mathbb{C}}
	\newcommand{\F}{\mathbb{F}}
	\newcommand{\Fc}{{\overline{\mathbb{F}}}}
	\renewcommand{\K}{\mathbb{K}}
	\renewcommand{\R}{\mathbb{R}}
	\newcommand{\N}{\mathbb{N}}
	\newcommand{\Ni}{\N\cup\infty}
	\newcommand{\bbP}{\mathbb{P}}
	\newcommand{\Q}{\mathbb{Q}}
	\newcommand{\Z}{\mathbb{Z}}

	% misc
	\newcommand{\e}{\mathrm{e}}
	\newcommand{\T}{t}
	\newcommand{\eps}{\epsilon}
	\newcommand{\hmu}{\hat{\mu}}
	\newcommand{\sle}{\preccurlyeq}

	\newcommand{\eqdef}{:=}
	\newcommand{\defeq}{=:}
	\renewcommand{\O}{\mathcal{O}}
	\newcommand{\ignore}[1]{}

	%Special charater types
	%	.	blackboard bold
	%	c	mathcal

	%	m	matrix
	%	r	random variable
	%	v	vector

	%matrices
	\newcommand{\mat}{}
	\newcommand{\mT}{\mat{T}}
	\newcommand{\mW}{\mat{W}}
	\newcommand{\mX}{\mat{X}}
	\newcommand{\mY}{\mat{Y}}
	\newcommand{\mZ}{\mat{Z}}

	\newcommand{\zmat}{\mathbf{0}}
	\newcommand{\Id}{\mathrm{I}}
	\newcommand{\zm}{\phantom{0}}
	\newcommand{\nulls}{\lambda}

	%random variables
	\newcommand{\rv}{\mathsf}

	% mathcal
	\newcommand{\cA}{\mathcal{A}}
	\newcommand{\cB}{\mathcal{B}}
	\newcommand{\cC}{\mathcal{C}}
	\newcommand{\cD}{\mathcal{D}}
	\newcommand{\cE}{\mathcal{E}}
	\newcommand{\cF}{\mathcal{F}}
	\newcommand{\cG}{\mathcal{G}}
	\newcommand{\cH}{\mathcal{H}}
	\newcommand{\cI}{\mathcal{I}}
	\newcommand{\cJ}{\mathcal{J}}
	\newcommand{\cK}{\mathcal{K}}
	\newcommand{\cL}{\mathcal{L}}
	\newcommand{\cM}{\mathcal{M}}
	\newcommand{\cN}{\mathcal{N}}
	\newcommand{\cO}{\mathcal{O}}
	\newcommand{\cP}{\mathcal{P}}
	\newcommand{\cQ}{\mathcal{Q}}
	\newcommand{\cR}{\mathcal{R}}
	\newcommand{\cS}{\mathcal{S}}
	\newcommand{\cT}{\mathcal{T}}
	\newcommand{\cU}{\mathcal{U}}
	\newcommand{\cV}{\mathcal{V}}
	\newcommand{\cW}{\mathcal{W}}
	\newcommand{\cY}{\mathcal{Y}}
	\newcommand{\cX}{\mathcal{X}}
	\newcommand{\cZ}{\mathcal{Z}}

	% named hitting sets
	\newcommand{\cHss}{\mathcal{H}^\text{ss}}
	\newcommand{\grinv}{\ensuremath{\cI^\mathrm{PRF}_{n,r}}}
	\newcommand{\invfs}{\ensuremath{\cI^\mathrm{FS}_{n,r}}}
	\newcommand{\invhitset}{\ensuremath{\cI^\cH_{n,r}}}
	\newcommand{\FS}{\text{FS}}

	% named prgs
	\newcommand{\prgnz}{\cG^\mathrm{nz}}

	\renewcommand{\vec}[1]{\overline{#1}}
	% vector mathcal
	\newcommand{\cvG}{{\vec{\cG}}}
	
	% lowercase random variables
	%\newcommand{\ra}{\rv{a}}
	\newcommand{\rb}{\rv{b}}
	\newcommand{\rc}{\rv{c}}
	\newcommand{\rd}{\rv{d}}
	\newcommand{\re}{\rv{e}}
	\newcommand{\rf}{\rv{f}}
	\newcommand{\rg}{\rv{g}}
	\newcommand{\rh}{\rv{h}}
	\newcommand{\ri}{\rv{i}}
	\newcommand{\rj}{\rv{j}}
	\newcommand{\rk}{\rv{k}}
	\newcommand{\rl}{\rv{l}}
	%\newcommand{\rm}{\rv{m}}
	\newcommand{\rn}{\rv{n}}
	\newcommand{\ro}{\rv{o}}
	\newcommand{\rp}{\rv{p}}
	%\newcommand{\rq}{\rv{q}}
	\newcommand{\rr}{\rv{r}}
	\newcommand{\rs}{\rv{s}}
	\newcommand{\rt}{\rv{t}}
	\newcommand{\ru}{\rv{u}}
	%\newcommand{\rv}{\rv{v}}
	\newcommand{\rw}{\rv{w}}
	\newcommand{\ry}{\rv{y}}
	\newcommand{\rx}{\rv{x}}
	\newcommand{\rz}{\rv{z}}

	% uppercase random variables
	\newcommand{\rA}{\rv{A}}
	\newcommand{\rB}{\rv{B}}
	\newcommand{\rC}{\rv{C}}
	\newcommand{\rD}{\rv{D}}
	\newcommand{\rE}{\rv{E}}
	\newcommand{\rF}{\rv{F}}
	\newcommand{\rG}{\rv{G}}
	\newcommand{\rH}{\rv{H}}
	\newcommand{\rI}{\rv{I}}
	\newcommand{\rJ}{\rv{J}}
	\newcommand{\rK}{\rv{K}}
	\newcommand{\rL}{\rv{L}}
	\newcommand{\rM}{\rv{M}}
	\newcommand{\rN}{\rv{N}}
	\newcommand{\rO}{\rv{O}}
	\newcommand{\rP}{\rv{P}}
	\newcommand{\rQ}{\rv{Q}}
	\newcommand{\rR}{\rv{R}}
	\newcommand{\rS}{\rv{S}}
	\newcommand{\rT}{\rv{T}}
	\newcommand{\rU}{\rv{U}}
	\newcommand{\rV}{\rv{V}}
	\newcommand{\rW}{\rv{W}}
	\newcommand{\rY}{\rv{Y}}
	\newcommand{\rX}{\rv{X}}
	\newcommand{\rZ}{\rv{Z}}
	
	%random vector variables
	\newcommand{\rvx}{{\vec{\rv{x}}}}
	\newcommand{\rvy}{{\vec{\rv{y}}}}
	\newcommand{\rvz}{{\vec{\rv{z}}}}

	\newcommand{\rvT}{{\vec{\rv{T}}}}
	\newcommand{\rvU}{{\vec{\rv{U}}}}
	\newcommand{\rvW}{{\vec{\rv{W}}}}
	\newcommand{\rvX}{{\vec{\rv{X}}}}
	\newcommand{\rvY}{{\vec{\rv{Y}}}}
	\newcommand{\rvZ}{{\vec{\rv{Z}}}}

	%vectors
	%need extra {} so that \vx^\va doesn't cause problems
	%use \ifnextchar to ensure that \vy^\va typesets with extra space to deal with the vector arrows, see https://tex.stackexchange.com/questions/16466/vector-arrow-with-superscript
	\makeatletter
	\newcommand{\va}{{\vec{a}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vb}{{\vec{b}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vc}{{\vec{c}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vd}{{\vec{d}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\ve}{{\vec{e}}\@ifnextchar{^}{\!\:}{}}
	%\newcommand{\vf}{{\vec{f}}\@ifnextchar{^}{\!\:}{}}
	%\newcommand{\vf}{{\vec{f}}\@ifnextchar{_}{\!\:\!}{}}
	\newcommand{\vf}{{\vec{f}}}
	%TODO: fix spacing, so that \vf \vf_i^n and \vf^n all look nice
	\newcommand{\vg}{{\vec{g}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vh}{{\vec{h}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vi}{{\vec{i}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vj}{{\vec{j}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vk}{{\vec{k}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vl}{{\vec{\ell}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vm}{{\vec{m}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vn}{{\vec{n}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vo}{{\vec{o}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vp}{{\vec{p}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vq}{{\vec{q}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vr}{{\vec{r}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vs}{{\vec{s}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vt}{{\vec{t}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vu}{{\vec{u}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vv}{{\vec{v}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vw}{{\vec{w}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vy}{{\vec{y}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vx}{{\vec{x}}\@ifnextchar{^}{}{}}		%\vec{x} seems fine already
	\newcommand{\vz}{{\vec{z}}\@ifnextchar{^}{\!\:}{}}

	\newcommand{\vA}{{\vec{A}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vB}{{\vec{B}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vC}{{\vec{C}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vD}{{\vec{D}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vE}{{\vec{E}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vF}{{\vec{F}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vG}{{\vec{G}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vH}{{\vec{H}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vI}{{\vec{I}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vJ}{{\vec{J}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vK}{{\vec{K}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vL}{{\vec{L}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vM}{{\vec{M}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vN}{{\vec{N}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vO}{{\vec{O}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vP}{{\vec{P}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vQ}{{\vec{Q}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vR}{{\vec{R}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vS}{{\vec{S}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vT}{{\vec{T}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vU}{{\vec{U}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vV}{{\vec{V}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vW}{{\vec{W}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vY}{{\vec{Y}}\@ifnextchar{^}{\!\:}{}}
	\newcommand{\vX}{{\vec{X}}\@ifnextchar{^}{}{}}		%\vec{x} seems fine already
	\newcommand{\vZ}{{\vec{Z}}\@ifnextchar{^}{\!\:}{}}
	\makeatother

	%greek vectors vectors
	\newcommand{\vaa}{{\vec{\alpha}}}
	\newcommand{\vbb}{{\vec{\beta}}}
	\newcommand{\vcc}{{\vec{\gamma}}}
	\newcommand{\vdd}{{\vec{\delta}}}
	\newcommand{\voo}{{\vec{\omega}}}
	\newcommand{\vsss}{{\vec{\sigma}}}

	%measures/sizes/norms
	\newcommand{\ellzero}[1]{{\ensuremath{\|#1\|_0}}}
	\newcommand{\ellone}[1]{{\ensuremath{\|#1\|_1}}}
	\newcommand{\ellinfty}[1]{{\ensuremath{\|#1\|_\infty}}}
	\newcommand{\elltimes}[1]{{\ensuremath{\|#1\|_\times}}}


	%OLD: need to transition to new use of \ind

	%Recent latex learnings
	%\qedhere for putting \qed on last line of equation
	%\autoref for putting contexted references
	%\uline for underlining, it line breaks
	%\S for section symbol
	%\nameref to reference name of section, needs nameref package
	%\xspace in the command instead of "\ "
	%\texorpdfstring{pdf}{txt} for dealing with hyperref bookmarks https://tex.stackexchange.com/questions/53513/hyperref-token-not-allowed
	%clip art
	%	http://www.pdclipart.org/
	%	http://www.clker.com/
	%	http://openclipart.org/

	%conventions
	%	labels
	%		position
	%			\begin{ENV}\label{LABEL}
	%			\end{ENV}
	%		choice of label
	%			defn
	%			rmk
	%			q (question)
	%			constr
	%			ex
	%			res
	%				includes (as exact choice of result type can change
	%					prop
	%					lem
	%					thm - something quite non-trivial
	%					cor - anything that really follows quickly from othe rstuff
	%					clm - sometime that is very specific part of another result, cannot stand on its own, and inherits notation from the result
	%	defn
	%		thing being defined is in bold
	%	a,b,c,d,e,i,j,k for integers
	%	\alpha,\beta,\gamma for field constants
	%	\e for base of exponential



